Obfuscation Resilient Search through Executable Classification

Android applications are usually obfuscated before release, making it difficult to analyze them for malware presence or intellectual property violations. Obfuscators might hide the true intent of code by renaming variables and/or modifying program structures. It is challenging to search for executables relevant to an obfuscated application for developers to analyze efficiently. Prior approaches toward obfuscation resilient search have relied on certain structural parts of apps remaining as landmarks, un-touched by obfuscation. For instance, some prior approaches have assumed that the structural relationships between identifiers are not broken by obfuscators; others have assumed that control flow graphs maintain their structures. Both approaches can be easily defeated by a motivated obfuscator. We present a new approach,Macneto, to search for programs relevant to obfuscated executables leveraging deep learning and principal components on instructions. Macneto makes few assumptions about the kinds of modifications that an obfuscator might perform. We show that it has high search precision for executables obfuscated by a state-of-the-art obfuscator that changes control flow. Further, we also demonstrate the potential of Macneto to help developers understand executables, where Macneto infers keywords (which are from the relevant unobfuscated program) for obfuscated executables.

==> Makefile <==
# $Id: Makefile 1833 2006-06-19 21:51:36Z witchel $

.SUFFIXES: .fig .dvi .ps .pdf

VERSION = 0.0

#----------------------------------------------------------------------
# Source files.  Edit these variables for each new paper.
#----------------------------------------------------------------------

name = macneto

all: pdf bib

#----------------------------------------------------------------------
# LaTeX commands.
#----------------------------------------------------------------------

%.dvi:%.tex
	pdflatex $<

dvi: $(name).tex *.tex
	pdflatex $<

rub: $(name).tex 
	rubber -Wrefs -Wmisc $(name)

twice:
	pdflatex $(name)
	pdflatex $(name)

bib:
	bibtex $(name)
	pdflatex $(name)
	pdflatex $(name)


latex_junk = 	$(name).dvi \
		*.aux \
		*.log \
		$(name).blg \
		$(name).toc \
		$(name).out \
		psfig.aux \
		*.bbl \
		*.pdfsync

#----------------------------------------------------------------------
# Postscript/PDF generation.
#----------------------------------------------------------------------

$(name).ps:
ps: $(name).dvi *.tex
	latex $(name).tex && latex $(name).tex
	$(DVIPS) -P pdf -t letter -o $(name).ps $(name).dvi

summary: summary.dvi

#DVIPS = dvips
DVIPS = dvips

%.ps:%.dvi
	$(DVIPS) -P pdf -t letter -o $@ $<

%.ps2:%.dvi
	$(DVIPS) -t letter -o ps2.tmp -p 2 $<
	mpage -2 -P ps2.tmp > $@
	rm ps2.tmp

pdf: 
	pdflatex $(name).tex

# DISTILL = distill
DISTILL_FLAGS = -embedallfonts on -maxsubsetpct 100

DISTILL = ps2pdf
#DISTILL_FLAGS =

%.pdf:%.ps
	$(DISTILL) $(DISTILL_FLAGS) $<

#----------------------------------------------------------------------
# Document previewers.
#----------------------------------------------------------------------

x:
	xdvi -s 5 $(name) &

gv: $(name).ps
	ghostview $(name).ps &


# Garbage files.
junk = $(latex_junk) *.ps *.pdf *.out


#----------------------------------------------------------------------
# Miscellaneous.
#----------------------------------------------------------------------

tags:
	etags $(latex_files)

clean:
	rm -f $(junk)

count:
	wc $(latex_files)


==> mt.tex <==
\section{Implementation}
%\subsection{Topics in Machine Code}
\label{sec:mt}
%this section is now very redundant with the previous section.
%intro of topic modeling in software engineering tasks
Topic modeling \cite{Blei:lda} is a generative model that identifies the probabilities/memberships that a document has to (hidden) topics or groups.
Topic modeling has been widely used in the software engineering community to understand programs and detect anomaly \cite{Savage:2010:TET:1912607.1913324, Gorla:2014:CAB:2568225.2568276}.
Most existing software engineering approaches apply topic modeling on \textit{human descriptions} of programs or program documents to identify hidden topics from programs.
Instead of focusing on human words in programs, we propose to mine hidden topics from \textit{machine code} directly.
%In this paper, we even show that topic modeling on machine code can help developers deobfuscate programs.

%what is the state-of-the-art using topic modeling in the community and their drawbacks
Most existing topic modeling-based approaches to deobfuscation work by analyzing method names, comments or texts in source code.
In other words, these approaches treat each program as plain text and use topic modeling to identify topics in programs, as labeled by human words.
Our insight here is that these human words may be noisy and inaccurate to describe programs.
For example, an obfuscated or anonymized program may not have a meaningful method name or other identifiers, and would not have any comments left.
Existing approaches reliant on human words to cluster or classify programs by topics may fail to process such method.
%Further, programs have their own word set (instructions) and different structures with human documents.

%Our insight of using topic modeling on machine code
Instead of extracting program topics from human words (source code), we propose the concept of \textit{Machine Topics}, where we attempt to identify the probability distribution that a method belongs to multiple topics from \textit{machine code}.
In addition to considering the machine code in a single method, we penetrate the method by including machine code from its callees to understand the behavior/semantics of that method completely.
%Based on the idea of machine topics, we develop \theSystem, which deobfuscates programs by observing machine topics they exhibit.
Modeling instructions (machine code) as terms and methods in documents, \theSystem uses Latent Dirichlet Allocation \cite{Blei:lda} to extract hidden machine topics in methods.
To the best of our knowledge, \theSystem is the first system to identify topics of programs from machine code. 

\subsection{From Apps to Instruction Distributions}
\label{subsubsec:inst}
We use the instruction distribution of methods to abstract and approximate program behavior.
For each method, we summarize its instruction distribution by observing and computing the frequencies of important instructions.
The instruction distribution of a method, $M_{j}$, can be represented as $M_{j} = [freq_{j}^{I_{1}}, freq_{j}^{I_{2}},...freq_{j}^{I_{a}}]$, where $a$ represents the index of an instruction and $freq_{j}^{I_{a}}$ represents the frequency of the $a_{th}$ instruction in the method $M_{j}$.
\sysName considers various bytecode operations as individual instructions (e.g. loading or storing variables), as well as a variety of APIs provided by the Android framework.
To avoid over-specialization, \sysName groups very similar instructions together and represents them with a single word, for instance, considering all instructions for adding two values to be equivalent, abstracting away the difference between instructions for adding floating point numbers and instructions for adding integers.
Similarly, \sysName groups together Android APIs by package for its topic API.

\begin{table}
\centering
\setlength{\tabcolsep}{1pt}
\caption{\tablecap{The potential instructions marked as taint sources/sinks by \theSystem.}}
\begin{tabular}{lp{6.5cm}}
\toprule
\textbf{Opcode} & \textbf{Description}\\
\midrule
\texttt{xaload} & Load a primitive or an object from an array, where \texttt{x} represents a type of primitive or object. \\
\texttt{xastore} & Store a primitive or an object to an array, where \texttt{x} represents a type of primitive or object. \\
\texttt{arraylength} & Retrieve the length of an array. \\
\texttt{xadd} & Add two primitives on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{xsub} & Subtract two primitives on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{xmul} & Multiply two primitives on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{xdiv} & Divide two primitives on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{xrem} & Compute the remainder of two primitives on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{xneg} & Negate a primitive on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{xshift} & Shift a primitive on the stack, where \texttt{x} represents integer or long. \\
\texttt{xand} & Bitwise-and two primitives on the stack, where \texttt{x} represents integer or long. \\
\texttt{xor} & Bitwise-or two primitives on the stack, where \texttt{x} represents integer or long. \\
\texttt{x\_xor} & Bitwise-xor two primitives on the stack, where the first \texttt{x} represents integer or long. \\
\texttt{iinc} & Increment an integer on the stack. \\
\texttt{xcomp} & Compare two primitives on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{ifXXX} & Represent all \texttt{if} instructions. Jump by comparing value(s) on the stack.\\
\texttt{xswitch} & Jump to a branch based on the index on the stack, where \texttt{x} represents \texttt{table} or \texttt{lookup}.\\
\texttt{android\_apis} & The APIs offered by the Android framework, which usually starts from \texttt{android.}, \texttt{dalvik.}, \texttt{java.}. \theSystem records 235 android apis.\\
\bottomrule
\end{tabular}
\label{tab:insts}
\end{table}

Instead of solely considering the instructions directly in a method, we also merge the instructions from the callee method(s) that it invokes (recursively), which helps us understand program semantics thoroughly.
For constructing callgraphs for applications and libraries, we use FlowDroid \cite{Arzt:2014:FPC:2594291.2594299}, a state-of-the-art tool that computes static data and control flow.
%In a callgraph, a node is a method and each out-edge of it is the possible callee methods.

As an example: consider the method \texttt{readAndSort} and its corresponding callgraph, as shown in Figure \ref{fig:callgraph}.
\texttt{readAndSort} simply reads the first line of a file as a string and then sorts this string.
It delegates its functionality to two subroutines, \texttt{readFile} and \texttt{sort}.
Both \texttt{readFile} and \texttt{sort} also invoke several methods, such as \texttt{toCharArray} and \texttt{readLine} APIs included in Android to help them complete their tasks.

Given a method, \theSystem classifies its callee methods in two ways as follows:
\begin{itemize}
	\item Android: Android methods (APIs) are offered by the Android framework directly.
	\theSystem models these methods as single instructions as outlined above.
	\texttt{readLine} and \texttt{toCharArray} in Figure \ref{fig:callgraph} belong to this category.
	\item Application: Application methods are all methods beside the Android APIs.
	An application method can be from an application or be from the third party libraries used by an application.
	While \sysName treats Android APIs as individual instructions, any other method call is inlined into the calling method, resulting in the instruction distributions of those callee methods being merged directly in the current method.
\end{itemize}
We can then define the instruction distribution of a method as
\begin{equation}
	M_{j} = M_{j} + \sum_{k \in callees(M_{j})} M_{k}
	\label{eq:dist}
\end{equation}
, where $j$ is the index of the current method and $k$ represents the indices of its callee methods.
%These instructions distributions becomes a direct semantic representation of programs, while we treat those human texts such as method names and variable names as indirect decriptions.
We will then use these instruction distributions as the input source for next step to identify topics embedded in programs.

\xxx[jon]{I have a really tough time parsing the next sentence and can't fix it without knowing better what to write}
\xxx[mike]{Rewrite this section, give definitions and examples. Hope it is clearer.}
Some obfuscators may inject additional instructions into the original methods, which might then change the perceived semantics of those methods.
In particular, since \sysName inlines application method calls, inserting additional method calls could cause significant distortions to the instruction distribution of a method.
\sysName combats this obfuscation by learning (and then filtering out) superfluous method calls that are systematically inserted by obfuscators from the callgraphs before/after obfuscation of the same method.
We call this learning module on callgraphs as \emph{graph diff.}.
%Because \theSystem includes semantics from all callees of a method into itself, such semantic change may affect the effectiveness of deobfuscation.
%\theSystem equips with a callgraph difference analyzer to detect the instruction patterns from the injected methods inserted by the obfuscator.
For each method in an APK, \theSystem first analyzes the callee difference of the current method $M_{j}$ before and after the obfuscation 
\begin{equation}
	\Delta M_{j} = callees(M^{obfus}_{j}) - callees(M_{j})
\end{equation}
, where $callees(M_{j})$ and $callees(M^{obfus}_{j})$ represent the callees of $M_{j}$ before and after the obfuscation, respectively.
If $\Delta M_{j}$ is not empty, \theSystem records the instruction distributions of the methods in $\Delta M_{j}$ as patterns.
In a training APK set, \theSystem computes the appearances of each pattern (instruction distribution) it learns from the callee differences and reports those patterns having high support.
We first define the total callee differences detected by \theSystem as 
\begin{equation}
	Diff_{callee}(T) = \sum_{k} \Delta M_{k}
\end{equation}
, where $T$ represents a training APK set and $k$ is the method index.
Then we define the support of a pattern as 
\begin{equation}
\begin{split}
	Support(Pattern_{i}) = \frac{Count(Pattern_{i})}{\sum_{j} Count(Pattern_{j})}
\end{split}
\end{equation}
, where $i$ is pattern index, $Pattern_{i} \in Diff_{callee}(T)$ and $Count(.)$ returns the appearance number of a pattern.

We again use the \texttt{readAndSort} example in \reffig{fig:callgraph} to demonstrate how graph diff. works.
Assuming \texttt{readAndSort} is transformed by an obfuscator that injects a method \texttt{decrypt(String)} to decrypt string literals, the callees of \texttt{readAndSort} becomes $callee(M^{obfus}_{r\&s}) = \{\texttt{read}, \texttt{sort}, \texttt{decrypt}\}$.
Thus, the $\Delta M_{r\&s} = \{\texttt{decrypt}\}$.
The instruction distribution of \texttt{decrypt}, $M_{decrypt}$, is recorded by \theSystem as a pattern.
If the support of such pattern is higher than a threshold ($0.03$ in this paper), \theSystem report it as a significant pattern and uses it to filter out superfluous method calls in the testing APK set.
This step is optional in \theSystem, but can have positive impact to recover methods obfuscated by an advanced obfuscator, which will be discussed in Section \ref{sec:eval}.

\xxx{i think there needs to be more implementation details here. do we filter out some methods? how do we apply it to android, everything here is java? explain de-dexing, removing trivial methods, etc.}[jon]
\xxx{Add more implementation details here.}[mike]
For computing the instruction distribution for each method, we first convert APks to jars by Dex2Jar \cite{dex2jar}, read instructions from jars via a Java bytecode rewriting libarary ASM \cite{ASM} and then compute the instruction frequency.
In our training and testing phase in this paper, we filter out the trivial methods having instruction numbers $<30$ or instruction types $<10$, because they may not offer sufficient information for \theSystem to deobfuscate.

\begin{figure}
	\centering
	\begin{subfigure}[t]{.5 \textwidth}
		\lstinputlisting{code/main.txt}
		\includegraphics[scale=0.55]{fig/callgraph.eps}
	\caption{The \texttt{readAndSort} method and its callgraph.}
	\label{subfig:caller}
	\end{subfigure}
	~
	\begin{subfigure}[t]{.5 \textwidth}
		\lstinputlisting{code/calls.txt}
	\caption{The callee methods of \texttt{readAndSort}.}
	\label{subfig:callee}
	\end{subfigure}%
	\caption{The \texttt{readAndSort} method and its callgraph (a). Two callee methods, \texttt{readFile} and \texttt{sort}, of \texttt{readAndSort} (b).}
\label{fig:callgraph}
\end{figure}

\subsection{From Instruction Distributions to Machine Topics}
\label{subsec:i2m}
%Introduce and explain topic model
Latent Dirichlet Allocation (LDA) \cite{Blei:lda} is one of the most widely used topic models.
LDA models each document as a sequence of words, where each document can exhibit a mixture of different topics.
Each topic is modeled as a distribution of words.
Thus a topic, $T_{j}$, can also be represented by a vector containing the word distribution $T_{i} = [Pr_{i}^{W_{1}}, Pr_{i}^{W_{2}}...Pr_{i}^{W_{a}}]$, where $i$ is the topic index and $Pr_{i}^{W_{a}}$ represents the probability that $T_{i}$ can have the word $W_{b}$.
A document, $D$, can be represented by a vector containing the topic distribution $D_{j} = [Pr_{j}^{T_{1}}, Pr_{j}^{T_{2}}...Pr_{j}^{T_{b}}]$, where $i$ is the document index and $Pr_{j}^{T_{b}}$ represents the probability that $D_{j}$ exhibits the topic $T_{b}$.
Both $D_{i}$ and $T_{j}$ are modeled as Dirichlet Distributions.

%What is machine topic?
Following the concept of LDA, we model a \textit{machine topic} as a machine word (instruction) vector 
\begin{equation}
	MT_{i} = [Pr_{i}^{I_{1}}, Pr_{i}^{I_{2}}...Pr_{i}^{I_{a}}]
	\label{eq:mt}
\end{equation}
, where $MT_{i}$ is the $i_{th}$ machine topic and $Pr_{i}^{I_{a}}$ represents the probability that the $a_{th}$ machine word (instruction) exists in $MT_{i}$.
The binary of each program (method) can be modeled as a machine topic vector (MTV)
\begin{equation}
	MTV(M_{j}) = [Pr_{j}^{MT_{1}}, Pr_{j}^{MT_{2}}...Pr_{j}^{MT_{b}}]
	\label{eq:method}
\end{equation}
, where $M_{j}$ represents the $j_{th}$ method and $MT_{b}$ represents the $b_{th}$ machine topic.
In \theSystem, we define $35$ machine topics ($a = 35$) and have $235$ types of instructions ($b = 252$) as we listed in \reftable{tab:insts}.
\xxx{where does 35 come from? it's configurable, right? does this mean we can only predict 35 different identifiers?}
While optimizing the topic number is out of the scope of this paper, we observe that $35$ machine topics can split all methods in a reasonable way
Please note that $35$ machine topics does not mean that there are solely $35$ classifications in \theSystem.
A machine topic vector/distribution forms a classification, so there can be infinite classifications (``shape'' of distributions) in \theSystem in theory.
To compute machine topics and topic vector for each method, we use the Mallet library \cite{mallet}.

%Why machine topic is a better characterization of programs, compared with those approaches using human words
%Machine topics offer an effective and less sensitive approach to automatically characterizing programs that have similar semantics and behaviors regardless of whether they share similar program structures.
%While most approaches use human words, such as comments and identifiers, as the proxy to characterize programs, we assume that machine code can be a more direct characterization of programs.
%However, using machine code directly to characterize programs is too sensitive and offers negative results, which will be seen in our evaluation in Section \ref{sec:eval}.
%Based on machine code in programs, machine topic can tolerate differences in programs that do not affect program semantics, which offers a better characterization to support deobfuscation.

%Summarize machine topic, connect to learning
\theSystem uses the instruction distribution of a method, $M_{j}$, to infer its machine topic distribution, $MTV(M_{j})$.
$MTV$ then becomes the annotation of both $M_{j}$ and its obfuscated counter part $M^{obfus}_{j}$ to train our classifier in \theSystem, which will be discussed in Section \ref{sec:deob}.

\xxx{suspect there should be some more details here too but not sure what to ask for}[jon]

==> mt_gail.tex <==
\section{Machine Code $\Leftrightarrow$ Human Word}
\label{sec:mt}

\xxx{pdflatex does not allow this section title, produces errors like
Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 1.
}

\xxx{this is about program understanding, no mention of deobfuscation, I'm wondering again if I'm looking at the wrong paper.  is there intended to be an earlier section presenting deobfuscation as a program understanding problem? and in turn explaining the program understanding problem as a clustering problem?}

Most approaches that help developers understand programs focus on extracting and mining the \textit{text} patterns or topics from documents, method names and/or token identifiers from codebases.\xxx{need some citations for these ``most approaches''. also what is a token identifier, does this mean parameter, variable, constant, etc. names or something else?}
This implies that these approaches treat programs as documents and use their text information (human language) as a \textit{proxy} of programs' semantics. 

However, a program's text information can be sparse, e.g., the naming of a method including its method name and the tokens in its method body is not precise\xxx{what does precise mean here, an example may help}
and there may be no comments or other human language documentation.\xxx{cite someone who says this happens frequently in real-world code. }
Such a method may not be amenable to text-based approaches.\xxx{remind that this text information is intentionally missing or misleading in obfuscated code}

Further, one reason that programs may be harder for humans to understand than common documents is that programs are \textit{alive}:
In addition to the text information of the method itself, many other factors can affect the program semantics such as the external APIs and instructions it uses. \xxx{what about the human words used in programming language statements at the source code level like ``if'' and ``then''?  are these token identifiers as above?  these are arguably both text and instructions.} 

We developed \theSystem to bridge the gap between text information of programs described in human words and the machine semantics of programs encoded in instructions.\xxx{do we want to say something like In other words, we aim to try to recover the human words of obfuscated programs from the machine code.}
Programs having similar semantics share the same topic and should be clustered together.\xxx{why do we need clusters at all, what are the clusters used for? relevance to deobfuscation}
Instead of using text mining techniques, such as topic modeling \cite{Blei:lda}, to cluster programs based solely on their method names or documentation,
\theSystem applies topic modeling on machine language, the program instructions, to detect clusters among programs.
We call these clusters \textit{Machine Topics}.
The programs in the same machine topic share similar semantics at the level of machine code.

Based on these machine topics, \theSystem then attempts to learn the relationships between semantics in human words and machine code.
To be more specific, \theSystem learns the projection model to apply to codebases to convert machine code to human words, and vice versa.
An analogous conversion technique has been successfully applied to classify/predict unknown images to correct human descriptions corresponding to their pixel patterns \cite{SocherGMN13}.\xxx{this needs more explanation if the intent is to clarify what we mean by projection model and convert}

The high level procedure of \theSystem can be seen in Figure \ref{fig:main}.
Because \theSystem works on the level of machine code, each program is first compiled to an executable.\xxx{in the case of obfuscated malware, all we have is the executable}
In this paper, we use Java \cite{jvm-spec7}\xxx{shouldn't this be a citation of java spec 8 not spec 7? or a generic java  reference independent of version? or just don't cite at all, the readers know what java is} as the target language, so the executable here contains Java bytecode.


%Compared with the exsiting approaches that mostly map developers' queries to method names or variable names (human space), \theSystem first converts the queries in human language from developers to the space of machine code and then search for the closest programs.
We will discuss the details of each step in the following sections.

\xxx{pdflatex cannot handle .eps files}
\begin{figure*}[t]
	\centering
	\includegraphics[scale=0.6]{fig/main_obfus.eps}
	\caption{The system architecture of \theSystem, which includes two branches: program analysis to extract machine topics and text analysis to identify natural text topics from programs.}
	\label{fig:main}
\end{figure*}

\subsection{Instruction Distribution on Call Graphs}
For abstracting and approximating program behaviors, we use the instruction distributions of programs as proxies.
For each method, we summarize its instruction distribution by observing and computing the frequencies of some important instructions.
The instruction distribution of a method, $m$, can be represented as $Insts(m)=[f_{0}, f_{1},...f_{n}]$, where $n$ represents the index of an instruction and $f$ represents the frequency of the instruction $i$ in the method $m$.
Table \ref{tab:insts} includes the important instructions recorded by \theSystem.\xxx{why aren't *all* instructions recorded?  something akin to stop words?}

\begin{table}
\centering
\setlength{\tabcolsep}{1pt}
\caption{\tablecap{The potential instructions marked as taint sources/sinks by \theSystem.}}
\begin{tabular}{p{2.0cm}p{6.5cm}}
\toprule
\textbf{Opcode} & \textbf{Description}\\
\midrule
\texttt{xaload} & Load a primitive or an object from an array, where \texttt{x} represents a type of primitive or object. \\
\texttt{xastore} & Store a primitive or an object to an array, where \texttt{x} represents a type of primitive or object. \\
\texttt{arraylength} & Retrieve the length of an array. \\
\texttt{xadd} & Add two primitives on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{xsub} & Subtract two primitives on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{xmul} & Multiply two primitives on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{xdiv} & Divide two primitives on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{xrem} & Compute the remainder of two primitives on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{xneg} & Negate a primitive on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{xshift} & Shift a primitive on the stack, where \texttt{x} represents integer or long. \\
\texttt{xand} & Bitwise-and two primitives on the stack, where \texttt{x} represents integer or long. \\
\texttt{xor} & Bitwise-or two primitives on the stack, where \texttt{x} represents integer or long. \\
\texttt{x\_xor} & Bitwise-xor two primitives on the stack, where the first \texttt{x} represents integer or long. \\
\texttt{iinc} & Increment an integer on the stack. \\
\texttt{xcomp} & Compare two primitives on the stack, where \texttt{x} represents a type of primitive. \\
\texttt{ifXXX} & Represent all \texttt{if} instructions. Jump by comparing value(s) on the stack.\\
\texttt{xswitch} & Jump to a branch based on the index on the stack, where \texttt{x} represents \texttt{table} or \texttt{lookup}.\\
\texttt{android\_apis} & The APIs offered by the Android framework, which usually starts from \texttt{android.}, \texttt{dalvik.}, \texttt{java.}. \theSystem records 235 android APIs.\\
\bottomrule
\end{tabular}
\label{tab:insts}
\end{table}

\theSystem does not only consider the machine code used by the method, but also by its callee methods.
Thus we construct call graphs for each program, and merge the instructions from the callee method(s) it invokes into the method's instruction distribution.
%, which helps us understand program semantics thoroughly.
For constructing callgraphs for applications and libraries, we use FlowDroid \cite{Arzt:2014:FPC:2594291.2594299}, which computes static data flow to enhance the precision of callgraphs.
In a callgraph, each node is a method and each out-edge refers to a possible callee method.

An exemplary caller method \texttt{readAndSort} and its callgraph can be seen in Figure \ref{fig:callgraph}.
The \texttt{readAndSort} method reads the first line in a file as a string and then sorts this string.
It delegates its functionality to two callee methods, \texttt{readFile} and \texttt{sort}.
Both \texttt{readFile} and \texttt{sort} also invoke several callee methods, such as \texttt{toCharArray} and \texttt{readLine} offered by Android, to help them complete their tasks.

Given a method, \theSystem classifies its callee methods in two ways as follows:
\begin{itemize}
	\item Android: Android methods (APIs) are offered by the Android framework directly.
	\theSystem models these methods as single instructions as we discussed in Table \ref{tab:insts}.\xxx{it doesn't make any sense to ``discuss'' something in a table, should there be separate discussion in the prose?}
	\texttt{readLine} and \texttt{toCharArray} in Figure \ref{fig:callgraph} belong to this category.
	\item Application: Application methods are the callees other than Android APIs.
	An application method can be written within an application or be provided by a third party library used by this application.
	Given a method, instead of modeling the application methods it invokes as single instructions, \theSystem collects and merges the instruction distributions of these callee methods with the current method.
\end{itemize}
We can then define the instruction distribution of a method as
\begin{equation}
	Insts(m_{i}) = Insts(m_{i}) + \sum_{j} Insts(m_{j})
	\label{eq:dist}
\end{equation}
, where $i$ is the index of the current method and $j$ represents the indices of its callee methods.
%These instructions distributions becomes a direct semantic representation of programs, while we treat those human texts such as method names and variable names as indirect decriptions.
We will then use these instruction distributions of methods as the input source for next step, \textit{Machine Topic}, to identify topics embedded in programs.

\xxx{pdflatex cannot handle .eps files}
\begin{figure}
	\centering
	\begin{subfigure}[t]{.5 \textwidth}
		\lstinputlisting{code/main.txt}
		\includegraphics[scale=0.55]{fig/callgraph.eps}
	\caption{The \texttt{readAndSort} method and its callgraph.}
	\label{subfig:caller}
	\end{subfigure}
	~
	\begin{subfigure}[t]{.5 \textwidth}
		\lstinputlisting{code/calls.txt}
	\caption{The callee methods of \texttt{readAndSort}.}
	\label{subfig:callee}
	\end{subfigure}%
	\caption{The \texttt{readAndSort} method and its callgraph (a). Two callee methods, \texttt{readFile} and \texttt{sort}, of \texttt{readAndSort} (b).}
\label{fig:callgraph}
\end{figure}

\subsection{Machine Topics}
The main target of the machine topic analyzer in \theSystem is to extract the semantics of a group or cluster of programs directly from its instructions, in addition to its human descriptions.\xxx{remind that obfuscated code has no human description or perhaps has a bogus human description.}
These two types of semantics will then be used to learn the relation between machine code and human words, discussed in next section.

Programs with similar machine semantics may be described by different human words.\xxx{or by no human words?}
Thus, to observe the representative human descriptions for a cluster of programs having similar machine semantics, we first cluster programs based on their instruction distributions.
By modeling each method as a document and their \textit{instructions} as terms (words), we conduct topic modeling analysis \cite{Blei:lda} to cluster these methods.
While using topic modeling to cluster programs on source code has been applied by previous work \cite{icse:lda}, we believe we are the first to apply such text mining techniques on \textit{instructions}, the language of machines.
Our assumption is that the programming language itself is more direct than human language to represent semantics of programs.\xxx{this would argue for using the source code not the machine code, unless the paper also says something about there are many different ways in the same source programming language to represent what the compiler produces as the same machine code.}
Our model, \textit{Machine Topics}, offers a different point of view to group programs that have similar semantics or behaviors with existing approaches that work with method names and documents.\xxx{is *with* the right word here, we are grouping programs with similar executables into the same clusters with other programs that have been grouped based on their human words?}

The programs under the same machine topic share the similar \textit{machine semantics} and/or behavior.
We then extract important human terms from method names or method descriptions of these programs.\xxx{but above we say there aren't any human terms in the target programs. or do we mean that some of the programs have human words and some don't, so we borrow the human words from other programs in the same cluster to also describe those programs without human words? this is the identical approach to http://dl.acm.org/citation.cfm?doid=2986012.2986013, so must be cited/compared to here}
\notice{Masud can help describe his keyword extraction here}
We treat these important human terms as the \textit{human semantics} of these programs.

Based on both machine semantics and human semantics from programs under different machine topics, we can learn the relation/projection between these two types of semantics.\xxx{ don't we use the human words of programs in the same machine topic not a different machine topic?}
While machine semantics can be quantitatively represented by instruction distributions, human semantic is still described by the important human words.\xxx{why not also use the distribution?}
To represent these human words in a computational format such as vectors, we use the Word Embedding model in next section.

\subsection{Word Embeddings}
\notice{Mention that word embeddings is the model to quantitatively measure the distance between human words.}

\subsection{Deep Learning}
\notice{Talk about the neural network to convert programs to word space.}

\subsection{Query Model}
\notice{Give examples to show how developers can query programs from human words to machine words.}
\xxx{query is for the code search problem, what is the model for the deobfuscation problem?}

